Squared-Norm Empirical Process in Banach Space

This note extends a recent result of Mendelson on the supremum of a quadratic process to squared norms of functions taking values in a Banach space. Our method of proof is a reduction by a symmetrization argument and observation about the subadditivity of the generic chaining functional. We provide an application to the supremum of a linear process in the sample covariance matrix indexed by finite rank, positive definite matrices.

==> generic-chaining.tex <==
%!TEX root = ./squared-norm-process.tex
\begin{definition}
  Given a metric space $(T,d)$ and $A$ a subset of $T$, define the \emph{diameter} 
  of $A$ to be
  \begin{equation}
    \Delta(A) \coloneqq \sup_{t,u \in A} d(t,u)\,.
  \end{equation}
\end{definition}
\begin{definition}
  Given a metric space $(T,d)$ and $\mathcal{A}$ a partition of $T$,
  for $t \in T$, define $\mathcal{A}(t)$ to be the unique element of $\mathcal{A}$ 
  that contains $t$.
\end{definition}

\begin{definition}[{\textcite{Talagrand}}]
  Given a metric space $(T,d)$,
  an \emph{admissible sequence} is an increasing sequence 
    $(\mathcal{A}_s)_{s \geq 0}$ of partitions of $T$ such that $\card{\mathcal{A}_0} = 1$ 
    and, for $s \geq 1$, $\card{\mathcal{A}_s} \leq 2^{2^s}$.
  For $\alpha \geq 1$, define the $\gamma_\alpha$ functional by 
  \begin{equation*}
    \gamma_\alpha(T, d) 
    \coloneqq \inf \sup_{t \in T} \sum_{s \geq 0} 2^{s/\alpha} \Delta(\mathcal{A}_s(t))
    \,,
  \end{equation*}
  where the infimum is taken over all admissible sequences.
\end{definition}

\begin{lemma}
  \label{lem:generic-chaining-subadditivity}
  Let $(T, d)$ be a metric space and $T_1, T_2 \subseteq T$.
  Then
  \begin{equation*}
    \gamma_\alpha(T_1 \cup T_2, d) 
    \leq 
    3 d(T_1, T_2) + 4\gamma_\alpha(T_1, d) + 4\gamma_\alpha(T_2, d)
    \,.
  \end{equation*}
\end{lemma}
\begin{proof}
  Let $(\mathcal{A}_s)_{s \geq 0}$ be an admissible sequence for $T_1$ 
  such that
  \begin{equation}
    \label{eq:admissible-1}
    \sum_{s \geq 0} 2^{s/\alpha} \Delta(\mathcal{A}_s(t)) \leq 2 \gamma_\alpha(T_1, d) 
    \text{ for all $t \in T_1$},\,
  \end{equation}
  and $(\mathcal{B}_s)_{s \geq 0}$ an admissible sequence for $T_2$ 
  such that 
  \begin{equation}
    \label{eq:admissible-2}
    \sum_{s \geq 0} 2^{s/\alpha} \Delta(\mathcal{B}_s(t)) \leq 2 \gamma_\alpha(T_2, d) 
    \text{ for all $t \in T_2$}\,.
  \end{equation}
  We define partitions $\mathcal{C}_s$ of $T_1 \cup T_2$ as follows.  
  Let $\mathcal{C}_0 = \{ T_1 \cup T_2 \}$, 
  $\mathcal{C}_1 = \mathcal{C}_0$, 
  and, for $s \geq 2$, let $\mathcal{C}_s$ be the partition consisting of the 
  sets
  \begin{equation*}
    \label{eq:partition}
    \begin{gathered}
      A \cap (T_1 \setminus T_2) \text{ for $A \in \mathcal{A}_{s-2}$} \,, \\
      B \cap (T_2 \setminus T_1) \text{ for $B \in \mathcal{B}_{s-2}$} \,, \text{ and } \\
      A \cap B \text{ for $A \in \mathcal{A}_{s-2}$ and $B \in \mathcal{B}_{s-2}$} \,.
    \end{gathered}
  \end{equation*}
  It is straightforward to check that $(\mathcal{C}_s)_{s \geq 0}$ is an increasing 
  sequence of partitions of $T_1 \cup T_2$, 
  and that $\card{C_0} = \card{C_1} = 1$ and, for $s \geq 2$, 
  \begin{align*}
      \card{\mathcal{C}_s} 
    &\leq 
      \card{\mathcal{A}_{s-2}} + \card{\mathcal{B}_{s-2}}
      + \card{\mathcal{A}_{s-2}} \times \card{\mathcal{B}_{s-2}}
    \\
    &\leq
      2^{2^{s-2}} + 2^{2^{s-2}} + 2^{2^{s-1}}
    \leq
      2^{2^s}
    \,.
  \end{align*}
  Thus $(\mathcal{C}_s)_{s \geq 0}$ is an admissible sequence for $T_1 \cup T_2$.
  Let $t \in T_1 \cup T_2$.
  Since, for $s \geq 2$, every element of $\mathcal{C}_s$ is a subset of an element of 
  $\mathcal{A}_{s-2}$ and/or $\mathcal{B}_{s-2}$,
  \begin{align*}
      \sum_{s \geq 0} 2^{s/\alpha} \Delta(\mathcal{C}_s(t))
    &\leq
      3 \Delta(T_1 \cup T_2) 
      + \sum_{s \geq 2} 2^{s/\alpha} \Delta(\mathcal{C}_s(t))
    \\
    &\leq
      3 \Delta(T_1 \cup T_2)
      + \sum_{s \geq 0} 2^{s/\alpha} \Delta(\mathcal{A}_s(t))
      + \sum_{s \geq 0} 2^{s/\alpha} \Delta(\mathcal{B}_s(t))
    \\
    &\leq
      3
      \big[
        \Delta(T_1 \cup T_2) + \gamma_\alpha(T_1, d) + \gamma_\alpha(T_2, d)
      \big]
    \,,
  \end{align*}
  by \eqref{eq:admissible-1} and \eqref{eq:admissible-2}.
  Then 
  \begin{align*}
      \gamma_\alpha(T_1 \cup T_2, d)
    &\leq
      \sup_{t \in T_1 \cup T_2}
      \sum_{s \geq 0} 2^{s/\alpha} \Delta(\mathcal{C}_s(t))
    \\
    &\leq
      3 \big[
        \Delta(T_1 \cup T_2) + \gamma_\alpha(T_1, d) + \gamma_\alpha(T_2, d)
      \big]  
    \,.
  \end{align*}
  By the triangle inequality, for all $u_1 \in T_1$ and $u_2 \in T_2$ we have 
  \begin{align*}
    \Delta(T_1 \cup T_2)
    &= 
      \sup_{t_1, t_2 \in T_1 \cup T_2} d(t_1, t_2)
    \\
    &\leq 
      \sup_{t_1, t_2 \in T_1 \cup T_2} d(t_1, u_1) + d(u_1, u_2) + d(u_2, t_2)
    \\
    &\leq d(T_1, T_2) + \Delta(T_1) + \Delta(T_2) \\
    &\leq d(T_1, T_2) + \gamma_\alpha(T_1, d) + \gamma_\alpha(T_2, d) 
    \,.
  \end{align*}
  Thus,
  \begin{equation*}
      \gamma_\alpha(T_1 \cup T_2, d)
    \leq
      3 d(T_1, T_2) + 4 \gamma_\alpha(T_1, d) + 4 \gamma_\alpha(T_2, d)
      \,.
    \qedhere
  \end{equation*}
\end{proof}
